Adversarial Policies Beat Superhuman Go AIs

We attack the state-of-the-art Go-playing AI system KataGo by training adversarial policies against it, achieving a >97% win rate against KataGo running at superhuman settings. Our adversaries do not win by playing Go well. Instead, they trick KataGo into making serious blunders. Our attack transfers zero-shot to other superhuman Go-playing AIs, and is comprehensible to the extent that human experts can implement it without algorithmic assistance to consistently beat superhuman AIs. The core vulnerability uncovered by our attack persists even in KataGo agents adversarially trained to defend against our attack. Our results demonstrate that even superhuman AI systems may harbor surprising failure modes. Example games are available https://goattack.far.ai/.

==> sections/intro_old.tex <==
\section{Introduction (old)}
%
Reinforcement learning from self-play has achieved superhuman performance in a range of games including Go~\citep{silver2016}, chess and shogi~\citep{silver2016}, and Dota~\citep{openai2019dota}.
Moreover, idealized versions of self-play provably converge to Nash equilibria~\citep{brown1951,heinrich2015}.
Although realistic versions of self-play need not converge, their strong empirical performance seems to suggest this is rarely an issue in practice.

%
%
%
%

Nonetheless, prior work has found that seemingly highly capable continuous control policies trained via self-play can be exploited by \emph{adversarial policies}~\citep{gleave2020,wu2021}.
%
This suggests that self-play may not be as robust as previously thought.
However, although the victim agents are state-of-the-art for continuous control, they are still well below human performance.
%
This raises the question: are adversarial policies a vulnerability of self-play policies in general, or simply an artifact of insufficiently capable policies?

To answer this, we study a domain where self-play has achieved very strong performance: Go.
Specifically, we train adversarial policies end-to-end to attack KataGo~\citep{wu2019}, the strongest publicly available Go-playing AI system.
Using less than $14\%$ of the compute used to train KataGo,
we obtain adversarial policies that win >$99\%$ of the time against KataGo with no search, and >$97\%$ of the time against KataGo with enough search to be superhuman.
%

Critically, our adversaries do not win by learning a generally capable Go policy.
Instead, the adversaries trick KataGo into making serious blunders that result in KataGo losing the game (Figure~\ref{fig:cp505vis1-board}).
Despite being able to beat KataGo,
our adversarial policies lose against even amateur Go players (see Appendix~\ref{app:experiments:human-vs-adversary}). 
%
This is a clear example of non-transitivity, illustrated in Figure~\ref{fig:non-transitivity}.

%
%
%
%

Our adversaries have no special powers: they can only place stones or pass, like a regular player.
We do however give our adversaries gray-box access to the victim network they are attacking (Section~\ref{sec:threat-model}).
%
%
%
In particular, we train our adversaries using an AlphaZero-style training process~\citep{silver2018}, similar to that of KataGo.
The key differences are that we collect games with the adversary playing against the victim, and that we use the victim network to select victim moves during the \emph{adversary's} tree search.

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

KataGo can play at a strongly superhuman level, winning~\citep[Section~5.1]{wu2019} against ELF OpenGo~\citep{tian2019} and Leela Zero~\citep{pascutto2019} that are themselves superhuman.
In Appendix~\ref{app:experiments:strength}, we estimate that KataGo without search plays at the level of a top-100 European player, and that KataGo is superhuman at or above 128 visits of search per move.
Our attack scales far beyond this level, achieving a 72\% win rate against KataGo playing with $10^7$ visits of search per move.

%
%
%
%
%
%
%

%
%
%
%
%

%

Our paper makes three contributions.
First, we propose a novel attack method, hybridizing the attack of \citet{gleave2020} with AlphaZero-style training~\citep{silver2018}.
Second, we demonstrate the existence of two distinct adversarial policies against the state-of-the-art Go AI system, KataGo.
Finally, we provide a detailed empirical investigation into these adversarial policies, including showing they partially transfer to other Go AIs and learn interpretable strategies that can be replicated by experts under standard human playing conditions.
%
%
Our open-source implementation is available at \githuburl{}.
